DNN-based ensemble singing voice synthesis with interactions between singers

We propose a singing voice synthesis (SVS) method for a more unified ensemble singing voice by modeling interactions between singers. Most existing SVS methods aim to synthesize a solo voice, and do not consider interactions between singers, i.e., adjusting one's own voice to the others' voices. Since the production of ensemble voices from solo singing voices ignores the interactions, it can degrade the unity of the vocal ensemble. Therefore, we propose a SVS that reproduces the interactions. It is based on an architecture that uses musical scores of multiple voice parts, and loss functions that simulate the interactions' effect to acoustic features. Experimental results show that our methods improve the unity of the vocal ensemble.

==> tables/MOS_matomari.tex <==
% \begin{table}[t]
%     \centering
%     \caption{MOS on unity of vocal ensemble.}
%     \label{table:MOS_matomari}
%     \vspace{-3mm}
%     \footnotesize
%     \begin{tabular}{c|c}
%         Method                  & MOS $\pm 95\%$ conf. $(\uparrow)$ \\ 
%         \hline
%         Baseline                & $3.13\pm0.19$\\ 
%         MT                      & $3.08\pm0.20$\\ 
%         MT$+$F0diff             & $2.60\pm0.21$\\ 
%         MT$+$Powdiff            & $3.16\pm0.19$\\ 
%         MT$+$F0diff$+$Powdiff   & $2.95\pm0.18$\\ 
%     \end{tabular}
%  \end{table}

% updated 
\begin{table}[t]
    \centering
    \caption{MOS on unity of vocal ensemble. \textbf{Bold} indicates the best score and significantly better than baseline with $p < 0.05$.}
    \label{table:MOS_matomari}
    \vspace{3mm}
    \footnotesize
    \begin{tabular}{c|c}\toprule
        Method                  & MOS $\pm 95\%$ conf. $(\uparrow)$ \\ 
        % \hline
        \midrule
        Baseline                & $3.10\pm0.14$\\ 
        MT                      & $3.22\pm0.14$\\ 
        MT$+$F0diff             & $2.92\pm0.14$\\ 
        MT$+$Powdiff            & $\textbf{3.31}\pm0.13$\\ 
        MT$+$F0diff$+$Powdiff   & $2.89\pm0.14$\\ \bottomrule
    \end{tabular}
    \vspace{-3mm}
 \end{table}

